Directed Chain Generative Adversarial Networks

Real-world data can be multimodal distributed, e.g., data describing the opinion divergence in a community, the interspike interval distribution of neurons, and the oscillators natural frequencies. Generating multimodal distributed real-world data has become a challenge to existing generative adversarial networks (GANs). For example, neural stochastic differential equations (Neural SDEs), treated as infinite-dimensional GANs, have demonstrated successful performance mainly in generating unimodal time series data. In this paper, we propose a novel time series generator, named directed chain GANs (DC-GANs), which inserts a time series dataset (called a neighborhood process of the directed chain or input) into the drift and diffusion coefficients of the directed chain SDEs with distributional constraints. DC-GANs can generate new time series of the same distribution as the neighborhood process, and the neighborhood process will provide the key step in learning and generating multimodal distributed time series. The proposed DC-GANs are examined on four datasets, including two stochastic models from social sciences and computational neuroscience, and two real-world datasets on stock prices and energy consumption. To our best knowledge, DC-GANs are the first work that can generate multimodal time series data and consistently outperforms state-of-the-art benchmarks with respect to measures of distribution, data similarity, and predictive ability.

==> Neural Directed Chain SDEs as Generator for Exotic Time Series (icml)/tex/conclusion.tex <==
\section{Conclusion}

We propose a novel time series generator, DC-GANs, motivated by the study of \citet{detering2020directed, ichiba2022smoothness} on directed chain SDEs (DC-SDEs). Compared to more complicated graph systems, we find from numerical examples that the directed chain systems exhibit promising ability in fitting time series of multimodal probability distributions. We prove in theory that DC-GANs have the same flexibility as the Neural SDEs in capturing marginal distributions, and DC-GANs naturally embrace the non-Markovian property in the topological structure, if needed. We also prove that the correlation of the generated path decays exponentially fast as the graph distance of the generated path from the original data becomes large under some mild assumptions, and hence, the lack-of-independence problem can be overcome by walking along the directed chain. We present four numerical examples, two synthetic datasets generated by the SDEs, and two real-world data of stock price and energy consumption, and show that DC-GANs have a better performance than SigWGAN, CTFP, Neural SDEs, TimeGAN and TTS-GAN, with the comparable independence property. {We remark that the DC-GANs algorithm can also work with irregular data (i.e., the sample paths may have data sampled on different time grids), which may happen in healthcare applications. }


{\bf Potential Societal Impact.} The proposed DC-GANs in this paper offer a fast and flexible generative adversarial network method for machine learning research areas, such as biology, economics, environmental science, finance, medicine, and more, where path-dependent analysis is critical. They have the potential to contribute to research areas where sequential data is scarce or missing. Furthermore, the strong predictive power of DC-GANs demonstrated in the energy consumption example (Example 4) can aid in the development of energy management and help reduce energy waste. As DC-GANs are primarily used to generate time-series data or sequential data, rather than fake faces, the usual negative social impact associated with creating fake social media accounts to spam would not be a concern in this context.

%The proposed DC-GANs in the paper offer a fast and flexible generative adversarial network method in the machine learning research areas such as biology, economics, environmental science, finance, medicine, and more, where path-dependent analysis is critical. They have the potential to contribute to research areas where the sequential data is scarce or missing. Moreover, the strong predictive power of DC-GANs demonstrated in the energy consumption example (Example 4) can aid in the development of energy management and help reduce energy waste. As DC-GANs are primarily used to generate time-series data or sequential data, rather than fake faces, the usual negative social impact associated with creating fake social media accounts to spam would not be a concern here.


% of particles are preferred nowadays

%We provide the following future research directions.
%\begin{enumerate}
%    \item Can we prove theoretical results to show that directed chain SDEs have strong potentials in estimating non-Markovian processes?
%    \item In the proof of Theorem \ref{thm:flexibility}, we show that there are infinitely many $V_0, V_1$ can matching marginal distributions. Then a natural questions is: what is the right choice of the neural network structure to represent $V_0, V_1$ such that the model has better performance?
%\end{enumerate}



==> Neural Directed Chain SDEs as Generator for Exotic Time Series (icml)/tex/exp.tex <==
\section{EXPERIMENTS}
We present the performance of the proposed DC-GANs on four different datasets, including stochastic opinion dynamics, network dynamics from neural science, and real-world stock data and energy consumption data. In all cases, we set $q=10$, i.e., ``walk'' along the chain for ten steps during the decorrelating phase. Other hyperparameters for neural network training can be found in Appendix~\ref{app:experiment} for details. The example implementation of DC-GAN is available at \url{https://github.com/mmin0/DirectedChainSDE}.

{\bf Benchmarks \& Evaluation.} The first two synthetic datasets are generated by SDEs, the third real-world data set of stock price time series was extracted from Yahoo Finance\footnote{\url{https://finance.yahoo.com/quote/GOOG?p=GOOG&.tsrc=fin-srch}.}, and the fourth real-world energy consumption data were obtained from Ireland's open data portal\footnote{\url{https://data.gov.ie/dataset?theme=Energy}.}. 
We compare our results by DC-GANs with SigWGAN, CTFP, Neural SDEs and Transformer-based TTS-GANs, and DC-GANs give much better accuracy under discriminative, predictive, and maximum mean discrepancy (MMD) metrics detailed below. We also provide independence metrics to show that our decorrelating and branching scheme can resolve the independence problem. {We also test over different discriminators, and show the flexibility of choosing the one that brings better performance or has a faster running time.}


%, \recheck{under comparable running time}. 


%The first two synthetic datasets are generated by SDEs, and we compare our results to the Neural SDE generator. For the third real-world data example of stock price time series, we benchmark our model with both Neural SDE and TimeGAN \citep{yoon2019time} on disciminative, predictive and maximum mean discrepancy (MMD) metrics. We also provide independence metrics to show that our decorrelating and branching scheme can resolve the independence problem.

\subsection{Metrics}


{\bf Marginal Distribution \& MMD.} 
For the first two examples, we plot histograms to compare their marginal distributions at several time stamps. To measure the goodness of fitting for time series, we use {maximum mean discrepancy} (MMD) induced by the expected signature given in \eqref{eq:sig_mmd}.
%see \citep{, kidger2021neural, ni2021sig} for more details.

{\bf Discriminative Metric.}
To quantitively measure the similarity between the fake data generated by DC-GANs and real data, we train a post-hoc time series classifier by optimizing a two-layer LSTM to discriminate original and fake sequential data. The fake data is labeled \textit{nonreal} and the original data is labeled \textit{real}. The worse discriminative ability of the post-hoc time series classifier implies the better performance of the time series generator. Our discriminative score is calculated as the absolute difference between 0.5 and predicting accuracy on testing data, thus a smaller score indicates a better generator.


{\bf Predictive Metric.}
Typically, a useful time series dataset contains temporal evolution information, and we can predict the future given past data. We expect that DC-GANs can capture this temporal dynamic property accurately from the original data. To this end, we train an auxiliary two-layer LSTM sequential predictor on the generated time series and test this post-hoc predictor on the original time series. The predictive score is calculated as the $L^1$ distance between predicted sequences and true sequences on testing data (the real data), with smaller scores for better generators.

{\bf Independence Metric.}
It is crucial for success to show that our algorithm can address the independence problem. As an independence metric, we use 
\begin{equation}
\label{eq:independence_score}
\rho(x, y) := \sup_{t\in[0,T]} \| \rho(x_t, y_t) \|_1,
\end{equation}
where $x, y\in L^2(\Omega\times[0,T], \RR^N)$ and $\rho(x_t, y_t)$ represents the cross-correlation matrix between random vectors $x_t, y_t$. Smaller $\rho(x, y)$ means less correlation between real data $x$ and generated data $y$. 

These metric scores are used to measure the algorithms' discriminative ability, predictive ability, and the distance and correlation between the generated data and the true distribution. A decrease in the metric score suggests an improvement in the quality of the generated data. Furthermore, the decrease in independence score is supported by Theorem~\ref{thm:dependence_decay} and Theorem~\ref{thm:dependence_decay_formal} in Appendix.

All experiments are run over ten different random seeds, and we report the mean and standard deviation (in the parentheses) for all metrics in Tables~\ref{tab:opinion}--\ref{tab:energy}. We give more details on how all these metrics are implemented in Appendix \ref{app:experiment_metrics}.
%\rh{mention that further details will be given in supplementary materials.}

\subsection{Example 1: Stochastic Opinion Dynamics}\label{sec:OpinionDyn}

We first consider stochastic opinion dynamics modeled by the following MV-SDE
\begin{equation*}
    \ud Y_t = -\bigg[ \int_\RR \varphi_\theta(\|Y_t - y\|)(Y_t-y) \;\mu_t(\mathrm{d} y) \bigg]\ud t + \sigma \ud W_t,
\end{equation*}
where $\varphi_\theta$ is a interaction kernel with $\theta_1, \theta_2 >0$,
\begin{align*}
    \varphi_\theta(r) = \left\{ \begin{array}{ll}
    \theta_1 \exp\bigg( -\frac{0.01}{1-(r-\theta_2)^2} \bigg),     & r>0, \\
       0,  & r\le 0,
    \end{array} \right.
\end{align*}
and $\mu_t = \text{Law}(Y_t)$ denotes the distribution of $Y_t$.  
One can interpret $\theta_1$ as a scale parameter that characterizes the intensity of the attraction between entities, and $\theta_2$ as the range parameter that determines the distance, within which an entity must be of one another in order to interact. This model is widely used in many disciplines, from flocking and swarming behaviors in biology (where $Y_t$ is the position) to public opinion evolution in social science (where $Y_t$ is the opinion towards a topic). We refer to \citet{motsch2014heterophilious} for further details. 

We choose $\theta_1 =6$, $\theta_2 =0.2$, $\sigma = 0.1$, $T = 1$, $\Delta t = 0.01$, and generate 8192 paths. The distribution $\mu_t$ is approximated by the empirical distribution of 8192 samples. These samples are used to produce the blue density in Figure~\ref{fig:opinion}, where a clear shift in distribution from unimodality to bimodality is observed. 

%their performance by comparing

%Here we compare with the neural SDEs method \citep{kidger2021neural}. Figure~\ref{fig:opinion} gives the comparison of the marginal distributions at $t = 0.1, 0.3, 0.5, 0.7, 0.9, 1.0$. One can see that the neural DC-SDEs method can accurately capture the bimodal distribution in general, but the neural SDE method not. When measured by MMD, the neural DC-SDEs gives 0.07 while the neural SDEs produces 0.12. Discriminative and independence metrics are displayed in Table~\ref{tab:opinion}. Although, the purely independent samples generated by neural SDE has smaller independence score, but neural DC-SDE generates fake samples with the same level independence. In this example, our model produces more accurate fake data without independence issues.

We first compare with the Neural SDEs method \citep{kidger2021neural}. Figure~\ref{fig:opinion} gives the comparison of the marginal distributions at $t = 0.1, 0.3, 0.5, 0.7, 0.9, 1.0$. One can see that DC-GANs can accurately capture the bimodal distribution in general, but the Neural SDE method can not. Under the MMD metric \eqref{eq:sig_mmd}, the discrepancy of DC-GANs is $0.07$, while the Neural SDEs give $0.12$. More comparisons with SigWGAN, CTFP, Neural SDEs and TTS-GAN under discriminative, MMD, and independence metrics are provided in Table~\ref{tab:opinion}. Our proposed DC-GANs have a smaller discriminative score, and an independence score comparable with the ones produced by the Neural SDE generator, SigWGAN, CTFP and TTS-GAN, all of which generate purely independent samples. Therefore, we conclude that DC-GANs can produce fake data closer to the real data without independence issues.

%They have comparable independence score, while neural DC-SDEs has a smaller variance for the indepence score and a smaller discriminative score. Although the purely independent samples generated by neural SDEs have smaller independence scores, the neural DC-SDEs generate fake samples with the same level of independence and a smaller standard deviation. 

%Opinion SDE describes public opinion evolution in social media platform by a Mckean-Vlasov type SDEs. 


\begin{table*}[ht]
\caption{Stochastic Opinion Dynamics (Example 1). The scores are computed for SigWGAN, CTFP, Neural SDEs, TTS-GAN and DC-GANs under different metrics. The numbers in the parenthesis are the corresponding standard deviations of each score. Note that a smaller value means a better approximation, which indicates the DC-GANs provide more accurate fake data with compared independence and running time.} \label{tab:opinion}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{cllll}
\toprule
Method  & Discriminative & MMD & Independence & Time (min) \\
\midrule
%TimeGAN         & 0.102(0.021) & 0.038(0.001)  \\
SigWGAN & 0.213 (0.01)   & 0.328 (0.004) & 0.009(0.004) & 6.55\\
CTFP &  0.131 (0.02)  & 0.281 (0.005) & 0.010(0.003) & 5.58 \\
Neural SDEs             &  0.045 (0.025) & 0.122 (0.003) & 0.007 (0.005) & 7.07\\
TTS-GAN & 0.127(0.014) & 0.176(0.003) & 0.008(0.003) & 15.6 \\
DC-GANs            & {\bf 0.028 (0.019)} & {\bf 0.07 (0.003)} & 0.009 (0.004) & 6.82   \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}




\subsection{Example 2: Stochastic FitzHugh-Nagumo Model}


FitzHugh-Nagumo model is a standard model from neuroscience \citep{baladron2012mean,reisinger2022adaptive}, used to describe the neurons' interacting spiking. Mathematically, for $N$ neurons and $P$ different neuron populations, and $i\in\{1,\dots,N\}$,  we denote by $p(i)=\alpha, \alpha\in\{1,\dots,P\}$ the population of $i$-th particle that belongs to. The state vector of neural $i$, $(X_t^{i, N})_{t\in[0,T]}=(V_t^{i,N}, w_t^{i,N}, y_t^{i,N})_{t\in[0,T]}$, satisfies the SDE, 
\begin{equation*}%\label{eq:FN_sde}
\begin{aligned}
    \ud X_t^{t, N} &= f_\alpha(t, X_t^{t, N})\ud t + g_\alpha(t, X_t^{t, N})\left[ \begin{array}{c}
         \ud W_t^i  \\
         \ud W_t^{i,y} 
    \end{array} \right] \\
    & \quad+ \sum_{\gamma=1}^P\frac{1}{N_\gamma}\sum_{j,p(j)=\gamma}\bigg( b_{\alpha\gamma}(X_t^{i,N}, X_t^{j,N})\ud t\\
    &\qquad + \beta_{\alpha\gamma}(X_t^{i,N}, X_t^{j,N})\ud W_t^{i,\gamma} \bigg),
\end{aligned}
\end{equation*}
where $V$ denotes a short, nonlinear elevation of membrane voltage, $w$ denotes a slower, linear recovery variable,
$N_\gamma$ denotes the number of neurons in the population $\gamma$. We defer more details about model description and  training data generation to Appendix \ref{app:experiment_details}. 

The FitzHugh-Nagumo system is an example of a relaxation oscillator, and exhibits a characteristic excursion in phase space, before the variables $V$ and $w$ relax back to their rest values. As a result, their distributions are typically multimodal distributed; see Figure~\ref{fig:fitzhugh-dist} in Appendix~\ref{app:experiment_details}.








%For $\gamma, \alpha \in \{1,\dots, P\}$, $I^\alpha(t):=I$, $\forall t\in[0,T]$, $\forall \alpha$ for some constant value $I$,
%$$f_\alpha(t, X_t^{i,N}) = \left[\begin{array}{c}
%     V_t^{i,N}-\frac{(V_t^{i,N})^3}{3}-w_t^{i,N} + I^\alpha(t)  \\
%     c_\alpha(V_t^{i,N} + a_\alpha - b_\alpha w_t^{i,N})  \\
%     a^\alpha_r S_\alpha(V_t^{i,N})(1-y_t^{i,N}) - a_d^\alpha y_t^{i,N}
%\end{array}\right],$$
%$$g_\alpha(t, X_t^{i,N}) = \left[ %\begin{array}{cc}
%    \sigma_{\mathrm{ext}}^\alpha & 0 \\
%    0 & 0 \\
%    0 & \sigma_\alpha^y(V_t^{i,N}, y_t^{i,N})
%\end{array} \right]$$
%and 
%$$b_{\alpha\gamma}(X_t^{i,N}, X_t^{j,N})=\left[ %\begin{array}{c}
%    -\Bar{J}_{\alpha\gamma}(V_t^{i,N}-V^{\alpha\gamma}_{\mathrm{rev}})y_t^{i,N}  \\
%    0 \\
%    0
%\end{array} \right],$$
%$$\beta_{\alpha\gamma}(X_t^{i,N}, X_t^{j,N}).$$
%Moreover,
%\begin{align*}
%    & S_\alpha(V_t^{i,N}) = \frac{T^\alpha_{\max}}{1+e^{-\gamma_\alpha(V_t^{i,N} - V_T^{i,N})}}, \\
%    & \mc{X}(y_t^{i,N}) = \mathds{1}_{y_t^{i,N}\in(0,1)} \Gamma e^{-\Lambda/(1-(2y_t^{i,N}-1)^2)},\\
%    &\sigma_\alpha^y(V_t^{i,N}, y_t^{i,N}) = \sqrt{a_r^\alpha S_\alpha(V_t^{i,N})(1-y_t^{i,N}) + a_d^\gamma y_t^{i,N}} \times \\
%    &\hspace{10em} \mc{X}(y_t^{i,N}),
%\end{align*}
%and $(W^i, W^{i,y}, W^{i,\gamma}), i=1,\dots,N$ are standard 3 dimensional Brownian motions and mutually independent.
%All other parameters will be stated in Appendix \ref{app:experiment}. 

% Darker color means smaller differences, and thus a better fitting. 

Figure \ref{fig:fitzhugh} depicts the differences of their joint marginal densities between generated time series and training (real) time series on channels $1$ and $3$ at $t=0.1, 0.3, 0.5, 0.7, 0.9, 1.0$. The darker the color the smaller the differences, thus the closer the distribution and indicating a better generator. It can be observed that DC-GANs produce less difference in joint marginal densities at multiple time stamps. Under discriminative, predictive, and MMD metrics, DC-GANs give better samples than SigWGAN, CTFP, Neural SDEs, and TTS-GAN consistently; see Table \ref{tab:fitzhugh}. In particular, fake samples produced by DC-GANs are almost indistinguishable for a two-layer LSTM classifier after exhaustive training. By the comparison using MMD, one can see that DC-GANs generate fake samples with distributions significantly closer to real data than the other three methods. The independence scores given by \eqref{eq:independence_score} are nearly indistinguishable.

%When measured by MMD, Neural DC-SDE gives 0.48 while neural SDE produces 1.07.



\begin{figure*}[ht]
\vspace{-.05in}
\centering
\subfloat[$t=0.1$]{\includegraphics[width=0.15\textwidth]{figures/fitzhugh/bad/0_1_hist2d.pdf}} 
\subfloat[$t=0.3$]{\includegraphics[width=0.15\textwidth]{figures/fitzhugh/bad/0_3_hist2d.pdf}}
\subfloat[$t=0.5$]{\includegraphics[width=0.15\textwidth]{figures/fitzhugh/bad/0_5_hist2d.pdf}} 
\subfloat[$t=0.7$]{\includegraphics[width=0.15\textwidth]{figures/fitzhugh/bad/0_7_hist2d.pdf}}
\subfloat[$t=0.9$]{\includegraphics[width=0.15\textwidth]{figures/fitzhugh/bad/0_9_hist2d.pdf}} 
\subfloat[$t=1.0$]{\includegraphics[width=0.15\textwidth]{figures/fitzhugh/bad/1_0_hist2d.pdf}} \\
\subfloat[$t=0.1$]{\includegraphics[width=0.15\textwidth]{figures/fitzhugh/good/0_1_hist2d.pdf}} 
\subfloat[$t=0.3$]{\includegraphics[width=0.15\textwidth]{figures/fitzhugh/good/0_3_hist2d.pdf}}
\subfloat[$t=0.5$]{\includegraphics[width=0.15\textwidth]{figures/fitzhugh/good/0_5_hist2d.pdf}} 
\subfloat[$t=0.7$]{\includegraphics[width=0.15\textwidth]{figures/fitzhugh/good/0_7_hist2d.pdf}}
\subfloat[$t=0.9$]{\includegraphics[width=0.15\textwidth]{figures/fitzhugh/good/0_9_hist2d.pdf}} 
\subfloat[$t=1.0$]{\includegraphics[width=0.15\textwidth]{figures/fitzhugh/good/1_0_hist2d.pdf}}
\vspace{-.1in}
\caption{Stochastic FitzHugh-Nagumo Model (Example 2). Figures (a)-(f) are generated by Neural SDEs, and Figures (g)-(l) are generated by DC-GANs. They show their joint marginal densities differences between estimated time series and real-time series on channels $1$ (Dim 1) and $3$ (Dim 3) at $t\in\{0.1, 0.3, 0.5, 0.7, 0.9, 1.0\}$. Darker color means a smaller difference, and thus a better fitting. One can observe that DC-GANs produce less difference in joint marginal densities at multiple time stamps.}
\label{fig:fitzhugh}
\end{figure*}

%The numbers in the parenthesis are the corresponding standard deviations of each score. 

%, indicating that DC-GANs provide more accurate fake data with compared independence and running time.

\begin{table*}[htbp]
\caption{Stochastic FitzHugh-Nagumo Model (Example 2). The scores are computed for SigWGAN, CTFP, Neural SDEs, TTS-GAN and DC-GANs under different metrics. Note that a smaller value means a better approximation. Parenthesized numbers are standard deviations. } \label{tab:fitzhugh}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{clllll}
\toprule
Method  & Discrimative & Predictive & MMD & Independence & Time (min) \\
\midrule
SigWGAN & 0.126 (0.04)  & 0.44 (0.001)  & 0.737 (0.01)& 0.0083(0.0024) & 9.63\\
CTFP & 0.275 (0.05)  & 0.501 (0.004) & 1.095 (0.02) & 0.0088(0.0023) & 6.88\\
Neural SDEs             &  0.20 (0.003) & 0.44 (0.000) & 0.97 (0.02) & 0.0085 (0.0023) & 8.25 \\
TTS-GAN & 0.258(0.02) & 0.45(0.001) & 0.96(0.04) & 0.0082(0.002) & 16.3 \\
DC-GANs             & \textbf{0.01 (0.009)} & \textbf{0.439 (0.000)} & \textbf{0.47 (0.02)} & 0.0085 (0.0027) & 8.13 \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}

%the joint density between Dim 1 and Dim 3  depicts

%Differences of Joint Density between Dim 1 and Dim 3.



%, indicating that DC-GANs provide more accurate fake data with compared independence and running time.

\subsection{Example 3: Stock Price Time Series (Real Data)}
\begin{table*}[!t h]
\caption{Stocks Price Time Series (Example 3). The scores are computed for SigWGAN, CTFP, TimeGAN, Neural SDEs, TTS-GAN and DC-GANs under different metrics. Note that a smaller value means a better approximation. Parenthesized numbers are standard deviations. } \label{tab:stock}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{clllll}
\toprule
Model  & Discriminative &  Predictive & MMD & Independence  & Time (min) \\
\midrule
SigWGAN & 0.183 (0.03)  & 0.060 (0.004)  & 0.121 (0.011) & 0.012(0.004)& 4.13 \\
CTFP & 0.256 (0.05)  & 0.138 (0.006) & 0.187 (0.009) & 0.013(0.005) & 6.40 \\
TimeGAN         & 0.102 (0.021) & 0.038 (0.001)   & 0.0220 (0.007) & 0.011 (0.005) & $>$660\\
Neural SDEs             & 0.085 (0.028) & 0.048 (0.001) & 0.0193 (0.008) & 0.011 (0.006) & 9.93\\
TTS-GAN & 0.093(0.022) & 0.041(0.001) & 0.023(0.007) & 0.010(0.004) & 19.2 \\
DC-GANs             & \textbf{0.045 (0.015)} & \textbf{0.036 (0.000)} & \textbf{0.0133 (0.005)} & 0.013 (0.006) & 9.53\\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}
The third example is Google stock prices from 2004 to 2019, extracted from Yahoo Finance. Sequences of stock prices are known as continuous time series data with unknown distributions, and can even be non-Markovian. Our data have six channels, volume and high, low, opening, closing, and adjusted closing prices. Among all, the first five channels are multimodal.
The combined discriminator \eqref{eq:combined_loss} (Neural CDE and $\mathrm{Sig\mbox{-}W}_1$) is used in GAN for this experiment, and we list the comparison results in Table \ref{tab:stock}. One can see that DC-GANs outperform SigWGAN, CTFP, TimeGAN, Neural SDEs and TTS-GAN under all three metrics. %, with a comparable independence score and running time. 

%\footnote{The data set was extracted from Yahoo Finance: \url{https://finance.yahoo.com/quote/GOOG?p=GOOG&.tsrc=fin-srch}.}

\subsection{Example 4: Energy Consumption Data (Real Data)}
We download the Energy Consumption data from Ireland's open data portal, and choose four electric and gas consumption time series from 02/2011–02/2013, where channels 1,3, and 4 exhibit multimodal features. We list the comparison results in Table \ref{tab:energy}, which shows consistent advantages of DC-GANs compared with other methods under different metrics as in previous examples. Notice that DC-GANs can be used with both Neural CDEs (NCDE) and Signature Wasserstein (SigW) discriminators, and in this example, DC-GANs with SigW as the discriminator present better performance and have a faster running time.


%DC-GANs outperform SigWGAN, CTFP, TimeGAN, and Nueral SDEs under all three metrics.

%\footnote{Data were downloaded from Ireland’s open data portal \url{https://data.gov.ie/dataset?theme=Energy}}

%indicating again that DC-GANs provide more accurate fake data.

\begin{table*}[!h t]
\caption{Energy Consumption Data from Ireland's open data portal (Example 4). The scores are computed for SigWGAN, CTFP, Neural SDEs, and DC-GANs under different metrics. Note that a smaller value means a better approximation. Parenthesized numbers are standard deviations.}
\label{tab:energy}
\vskip 0.15in
\begin{center}
\begin{small}
\begin{sc}
\begin{tabular}{lccccr}
\toprule
Method  & Discriminative & Predictive & MMD & Independence & Time(min) \\
\midrule

SigWGAN & 0.368 (0.09)  & 0.159 (0.002)  & 0.135 (0.006) & 0.022(0.007) & 9.47\\
  CTFP & 0.487 (0.01)  & 0.185 (0.001) & 0.558 (0.006) & 0.021(0.008) & 8.52 \\
 Neural SDEs        &   0.413 (0.06)  & 0.172 (0.004)  & 0.126 (0.004) & 0.022(0.006) & 9.73 \\
 TTS-GAN & 0.394(0.04) & 0.167(0.003) & 0.183(0.008) & 0.022(0.006) & 17.4\\
 DC-GANs (w/ NCDE)   &   {0.322 (0.12)}     &  {0.155 (0.006)} & {0.077 (0.003)} & 0.029(0.007) & 23.44  \\
 DC-GANs (w/ SigW)   &   {\bf 0.310 (0.09)}     &  {\bf 0.151 (0.008)} & {\bf 0.075 (0.003)} & 0.033(0.008) & 9.38  \\
\bottomrule
\end{tabular}
\end{sc}
\end{small}
\end{center}
\vskip -0.1in
\end{table*}


\subsection{Dependence Elimination \& Ablation Study.} To demonstrate the effectiveness of removing dependence in the {\it Decorrelating and Branching Phase} (Section~\ref{sec:generator}), we compare the independence score \eqref{eq:independence_score} with choices of $q=2$ (basic model) and $q=10$ (DC-GANs), and present the results in Table \ref{tab:independence_compare}. A smaller score indicates better independence. The large differences observed in all four experiments suggest that the proposed scheme significantly reduces correlation in the directed chain generator. We anticipate that this approach can be employed in other directed chain-related methods to effectively mitigate strong dependence on generated data.

%To study the effectiveness of the decorrelating and branching scheme, we compare the independence score (see Eq. \eqref{eq:independence_score}) between a baseline model (with $q= 2$) and our DC-GAN method (with $q = 10$). Additionally, we conduct an ablation study on the discriminator by comparing the performance of DC-GAN with that of a vanilla WGAN with an LSTM discriminator.

%Due to the page limit, both studies are deferred to Appendix \ref{app:experiment_ablation}.

%\subsection{Extra Experiments} \label{app:experiment_ablation}

%\paragraph{Effectiveness of the Decorrelating and Branching Scheme.} 


\begin{table*}[!h t]
    \caption{The comparison of independence scores between a basic model (with $q=2$) and DC-GANs (with $q=10$). A smaller score indicates better independence.}
    \label{tab:independence_compare}
    \vskip 0.15in
    \centering
    \begin{sc}
    \begin{tabular}{cllll} \hline
       Experiments  & Opinion (Exp.1) & Fitz-Nag (Exp.2) & Stock (Exp.3) & Energy(Exp.4)\\ \hline 
       $q=2$ (Basic) &0.078(0.013) & 0.052(0.009)& 0.130(0.024) & 0.119(0.017) \\
       $q=10$ (DC-GANs) & 0.009(0.004) & 0.0085(0.0027) & 0.013(0.006) & 0.033(0.008) \\ \hline
    \end{tabular}
    \end{sc}
\end{table*}

%\paragraph{Ablation Study.} We also perform an ablation study on the discriminator. In particular, for comparison, we use an ordinary LSTM as the discriminator and implement Wasserstein-GAN. The results are summarized below, which show that DC-GANs have better and faster performance. 

 We also conduct an ablation study on the discriminator by using an ordinary LSTM as the discriminator and implementing Wasserstein-GAN for comparison. The results, summarized in Table~\ref{tab:wgan}, indicate that DC-GANs (shown in Tables~\ref{tab:opinion}-\ref{tab:energy}) outperform Wasserstein-GAN with an LSTM discriminator in both accuracy and speed.


%Although Sig-WGAN provides the best performance, directed chain generator can be used with other choices of discriminators and produce reasonable results.


\begin{table*}[!h t]
\caption{The scores computed when the discriminator is replaced by an ordinary WGAN. Parenthesized numbers are standard deviations. Compared to Tables~\ref{tab:opinion}-\ref{tab:energy}, DC-GANs outperform Wasserstein-GAN with an LSTM discriminator in both accuracy and speed.}\label{tab:wgan}
\vskip 0.15in
    \centering
    \begin{sc}
    \begin{tabular}{clllll} \hline
       Experiments  & Discriminative & Predictive & MMD & Independence& Time (min) \\ \hline 
       Stoch. Opinion  & 0.041(0.016) & - & 0.123(0.004) & 0.008(0.003) & 19.5\\ %\hline
       FitzHugh-Nagumo & 0.09(0.01) & 0.441(0.000) & 0.66 (0.07) &  0.0083(0.0022) & 26.2 \\ %\hline
       Google Stock & 
0.082 (0.024) & 0.059 (0.002) & 0.0176 (0.006) & 0.010 (0.005)  & 20.85 \\ %\hline
       Energy Consumption & 0.343 (0.13) & 0.161(0.004) & 0.093 (0.004) & 0.024(0.004) & 21.17 \\ \hline
    \end{tabular}
    \end{sc}
\end{table*}


==> Neural Directed Chain SDEs as Generator for Exotic Time Series (icml)/tex/intro.tex <==
\section{INTRODUCTION}
%Neural ordinary differential equations, using neural networks to parameterize the vector fields of a differential equation, have become phenomenal after its introduction by \cite{chen2018neural}. Since then, the framework has been applied to and motivated  various lines of research. On top of work aiming to improve Neural ODEs \citep{quaglino2019snode,zhang2019anodev2,massaroli2020dissecting,hanshu2019robustness}, 
%\cite{li2020scalable} and \cite{tzen2019neural} generalized it to neural stochastic differential equations (Neural SDEs) by combining SDE from stochastic analysis, and provide adjoint equations for efficient training. \cite{kidger2020neural} designed neural controlled differential equations (Neural CDEs) for generating time series by integrating rough path theory \citep{lyons2007differential}. One advantage of introducing those mathematical concepts into the framework is the capability of providing mathematical proofs to justify its validity, and in turn to get a deeper understanding of the framework itself. Other examples integrating profound mathematical concepts includes using higher order of kernel mean embeddings to capture information filtration \citep{salvi2021higher},  solving high dimensional partial differential equations through backward stochastic differential equations \citep{han2018solving}, to name a few.


%Since then, such mathematical objects inspired machine learning structure for time series data analysis are attracting increasingly attention. For example, neural controlled differential equations (Neural CDEs, by \cite{kidger2020neural}) used the rough differential equation concept from rough path theory \citep{lyons2007differential}, neural stochastic differential equations (Neural SDEs, by \cite{li2020scalable, kidger2021neural}) adapts the fundamental mathematical object (stochastic differential equations) from stochastic analysis and financial mathematics field. One beauty of using these kind of structure is that we get a deeper understanding of the model and are able to provide mathematical proofs to show their ability. Other examples includes \cite{salvi2021higher} used higher order of kernel mean embeddings to capture information filtration, \cite{han2018solving} proposed an efficient deep learning solver for high dimensional partial differential equations through backward stochastic differential equations, to name a few.

Generative models are important to overcome the limitation of data scarcity, privacy, and costs. In particular, medical data are not easy to get, use or share, due to privacy; and financial time series data are inadequate due to their nonstationarity nature. Times-series generative models, instead of seeking to learn the governing equations
%stochastic differential equations (SDEs) 
from real data, aim to discover and learn data automatically, and output new data that plausibly can be drawn from the original dataset. Some existing infinite-dimensional generative adversarial networks (GANs) (e.g., \citet{kidger2021neural,li2022tts}) showed successful performance in unimodal time series datasets.
However, many real-world phenomena are multimodal distributed, e.g., data describing the opinion divergence in a community \citep{tsang2014opinion}, the interspike interval distribution \citep{sharma2018suppression}, and the oscillators’ natural frequencies \citep{smith2019chaos}. All these bring the necessity of developing new generative models for multimodal time series data.



%In the direction of characterizing real-world random phenomena, SDEs have been considered crucial tools for their greatly developed theory, the availability to provide probabilistic predictions, and more importantly, for being able to capture the temporal evolution. Famous examples include the Black-Scholes model for stock prices, the Stochastic Susceptible-Infected-Removed model in epidemiology, and the Langevin equation in statistical physics, etc.


  %from a brand new system of the stochastic differential equations,  

In this paper, we develop a novel time-series generator, named \emph{directed chain GANs} (DC-GANs), motivated by the formulation of DC-SDEs \citep{detering2020directed}. The drift and diffusion coefficients in DC-SDEs depend on another stochastic process, which we call the neighborhood process, with distribution required to be the same as the SDEs' distribution. Different from other GANs, which only use real data in discriminators, our proposed algorithm naturally takes the dataset as the neighborhood process, giving generators access to data information. This feature enables our model to outperform the state-of-the-art methods on many datasets, particularly for the situation of multimodal time-series data. 


%and this is actually the real data during training, into its coefficients. Intuitively this model should have great capability to learn the target time series distribution, since it gets access to the true data directly. Under the directed chain SDEs setup, one key requirement is that the distribution between neighborhood and the generated SDEs must be the same, which serves naturally as the training objective. This method has an independence problem \ref{prob:independence} as the generated data depends on real data, but we propose an easy solution to this problem and provide corresponding mathematical proofs to our approach.


%\textbf{Contribution.} Our contributions can be summarized as follows, 
%\begin{enumerate}
%\vspace{-5pt}
 %   \item We propose a novel generator for exotically distributed time series based on a recently developed mathematical tool, Directed Chain SDEs (cf. Definition~\ref{def:dc_sde}), and prove that any distribution that neural SDEs are capable of generating can be covered by our model (see Theorem~\ref{thm:flexibility}). To train our generator, we propose to use a combination of two type of discriminators: Sig-WGAN \citep{ni2021sig} and Neural CDEs \citep{kidger2020neural};
    
 %   \item We point out that data generated immediately from Neural DC-SDEs may be correlated, and propose an easy solution to this issue by walking along the directed chain in the path space for further steps (see Theorem~\ref{thm:dependence_decay}). Combining with branching the chain with different Brownian noises  enables our model to generate unlimited independent fake data;
    
 %   \item We test our algorithms in three different experiments and show that our model provides the best performance compared to the other two popular models, TimeGAN \citep{yoon2019time} and Neural SDEs \citep{kidger2021neural}.
    
%\end{enumerate}

\paragraph{Contribution.} We propose a generator for multimodal distributed time series based on DC-SDEs (cf. Definition~\ref{def:dc_sde}), and prove that our model can handle any distribution that Neural SDEs are capable of generating (see Theorem~\ref{thm:flexibility}). To train the generator, we propose to use a combination of two types of discriminators: Sig-WGAN \citep{ni2021sig} and Neural CDEs \citep{kidger2020neural}.
    
    We notice that data generated immediately from DC-GANs can be correlated, and propose an easy solution by walking along the directed chain in the path space for further steps (see Theorem~\ref{thm:dependence_decay}). Combining branching the chain with different Brownian noises  enables our model to generate unlimited independent fake data.
    
    We test our algorithms in four different experiments and show that DC-GANs provide the best performance compared to existing popular models, including SigWGAN \citep{ni2021sig}, CTFP \citep{deng2020modeling}, Neural SDEs \citep{kidger2021neural}, TimeGAN \citep{yoon2019time} and Transformer-based generator TTS-GAN \citep{li2022tts}.
   



\paragraph{Related Literature.}
Neural ordinary differential equations (Neural ODEs), introduced by \citet{chen2018neural}, use neural networks to parameterize the vector fields of ODEs and bring a powerful tool for learning time series data. Later, significant effort has been put into improving Neural ODEs, e.g., \citet{quaglino2019snode,zhang2019anodev2,massaroli2020dissecting,hanshu2019robustness}. In fact, incorporating mathematical concepts into the Neural ODEs framework can provide the capability of analyzing and justifying its validity, leading to a deeper understanding of the framework itself. For example, \citet{li2020scalable} and \citet{tzen2019neural} generalized the idea to neural stochastic differential equations (Neural SDEs), providing adjoint equations for efficient training. By integrating rough path theory \citep{lyons2007differential}, \citet{kidger2020neural} proposed neural controlled differential equations (Neural CDEs) {and \citet{morrill2021neural} proposed neural rough differential equations} for modeling time series. Other examples integrating profound mathematical concepts include using higher order kernel mean embeddings to capture information filtration \citep{salvi2021higher}, and solving high dimensional partial differential equations through backward stochastic differential equations \citep{han2018solving}, to name a few.

The closely related model to ours is the Neural SDEs by \citet{kidger2021neural}, which uses the Wasserstein GAN method to train stochastic diffusion evolving in a hidden space and gains great success in simulating time series data. Other successful GANs models for time-series data include \citet{cuchiero2020generative,tzen2019theoretical,deng2020modeling,kidger2021neural,li2022tts}; see \citet{brophy2022generative} for a recent review. Note that we find in the numerical experiments that the performances of Neural SDEs are limited in simulating multimodal distributed time series, e.g., as shown in Figure~\ref{fig:opinion} from the stochastic opinion dynamics (Example 1 in Section~\ref{sec:OpinionDyn}). 



%From theoretical point of views, 

The directed chain is one of the simplest structures in random graph theory, where each node on the graph represents a stochastic process and has interactions only with its neighbor nodes (Figure~\ref{fig:chain}). To our best knowledge, \citet{detering2020directed} initiated the study of the SDE system on the directed chains, followed by \citet{feng2020linear, feng2020linear0} for the analysis of stochastic differential games on such chains with (deterministic and random) interactions. 
Later on, more complicated graph structures are studied beyond directed chains. For example, \citet{lacker2021locally} analyzed particle behaviors where the interaction only happens between neighborhoods in an undirected graph, and proved Markov random fields property and constructed Gibbs measure on path space when interactions appear only in drift; \citet{lacker2022case} considered stochastic differential games on transitive graphs; \citet{carmona2022stochastic} studied games on a graphon which has infinitely many nodes. Despite numerous extensions, {we find that the directed chain structure, although simple but rich enough for generating multimodal time series.} 

From another viewpoint, DC-SDEs can be understood as the reverse direction of mimicking theorems \citep{gyongy1986mimicking}. The idea of ``mimicking" is that for a general SDE (even with path-dependence features), one can construct a Markovian one to mimic its marginal distribution; see \citet{brunick2013mimicking} for details on mimicking aspects of It\^{o} processes including the distributions of running maxima and running integrals. DC-SDEs work in the reverse direction: they can produce marginal distributions that are generated by Markovian SDEs (see Theorem~\ref{thm:flexibility} for a detailed statement). The benefit of using DC-SDEs, in particular in machine learning, is to have a more vital fitting ability by embedding data into a slightly more complicated system. 


%turn out to be suitable for doing the vice versa of mimicking problem by embedding data into the slightly more complicated system and getting stronger fitting ability. 



\begin{figure*}[ht]
%\vspace{.3in}
\centering
\subfloat[$t = 0.1$]{\includegraphics[width=0.15\textwidth]{figures/opinion/bad/0_1.pdf}} 
\subfloat[$t = 0.3$]{\includegraphics[width=0.15\textwidth]{figures/opinion/bad/0_3.pdf}}
\subfloat[$t = 0.5$]{\includegraphics[width=0.15\textwidth]{figures/opinion/bad/0_5.pdf}} 
\subfloat[$t=0.7$]{\includegraphics[width=0.15\textwidth]{figures/opinion/bad/0_7.pdf}}
\subfloat[$t=0.9$]{\includegraphics[width=0.15\textwidth]{figures/opinion/bad/0_9.pdf}} 
\subfloat[$t=1.0$]{\includegraphics[width=0.15\textwidth]{figures/opinion/bad/1_0.pdf}} \\
\subfloat[$t=0.1$]{\includegraphics[width=0.15\textwidth]{figures/opinion/good/0_1.pdf}} 
\subfloat[$t=0.3$]{\includegraphics[width=0.15\textwidth]{figures/opinion/good/0_3.pdf}}
\subfloat[$t=0.5$]{\includegraphics[width=0.15\textwidth]{figures/opinion/good/0_5.pdf}} 
\subfloat[$t=0.7$]{\includegraphics[width=0.15\textwidth]{figures/opinion/good/0_7.pdf}}
\subfloat[$t=0.9$]{\includegraphics[width=0.15\textwidth]{figures/opinion/good/0_9.pdf}} 
\subfloat[$t=1.0$]{\includegraphics[width=0.15\textwidth]{figures/opinion/good/1_0.pdf}}
\vspace{-.1in}
\caption{Marginal distributions of real data (blue) and generated data (red) from Example 1 (Stochastic opinion dynamics) at $t\in\{0.1, 0.3, 0.5, 0.7, 0.9, 1\}$ in Section~\ref{sec:OpinionDyn}. Figures (a)--(f) are generated by Neural SDEs, and Figures (g)--(l) are generated by DC-GANs. One can see from Figures (e) and (f) that Neural SDEs fail to capture the bimodal distribution.}
\label{fig:opinion}

\end{figure*}

==> Neural Directed Chain SDEs as Generator for Exotic Time Series (icml)/tex/model.tex <==
\section{PROPOSED METHOD: DC-GANs}
\label{sec:model}

In this section, we describe DC-GANs for generating multimodal distributed time series. Our method builds on the DC-SDEs with a straightforward idea: To find the (sub-) optimal solution of the generator, we implement a GAN model with the Neural DC-SDEs as the generator. For the discriminator, we use Neural CDEs \citep{kidger2021neural} and Sig-Wasserstein GAN \citep{ni2020conditional, ni2021sig}.


\subsection{Generator}\label{sec:generator}
To overcome the independence issue explained in Problem~\ref{prob:independence}, we design DC-GANs by two phases: 1) training and 2)  decorrelating and branching. The second phase will be utilized during testing. Both $V_0$ and $V_1$ in \eqref{eq:dc_sde} will be parameterized by multi-layers fully connected NNs. % neural networks. 



{\bf Training Phase.}
We set aside the independence problem and focus on finding the optimal coefficients $V_0$ and $V_1$ (together with the discriminator). Denote the training data by $\{\Tilde{X}(\omega_i)\}_{i=1}^M$, where each $\omega_i$ represents a realization of the randomness in the path space. We treat our training data $\{\Tilde{X}(\omega_i)\}_{i=1}^M$ as the neighborhood process $\Tilde{X}$ in \eqref{eq:dc_sde}. For each training path data $\Tilde{X}(\omega_i)$, we generate a DC-SDE path $X(\omega_i)$, according to the Euler scheme of \eqref{eq:dc_sde},
\begin{align}
    &X_{t_{j+1}}(\omega_i) \nonumber\\
    & = X_{t_j}(\omega_i) + V_0(t_j, X_{t_j}(\omega_i), \tilde X_{t_j}(\omega_i)) (t_{j+1} - t_j) \label{eq:dc_sde-simulation}\\
    & \hspace{12pt}+ V_1(t_j, X_{t_j}(\omega_i), \tilde X_{t_j}(\omega_i))(B_{t_{j+1}}(\omega_i)-B_j(\omega_i)), \nonumber
\end{align}
where $0 = t_0 \leq t_1 \leq \ldots \leq t_J = T$ is a partition on $[0,T]$, $\{B(\omega_i)\}_{i=1}^M$ are independent Brownian paths. 

Both the generated paths $\{X(\omega_i)\}_{i=1}^M$ and the training paths $\{\Tilde{X}(\omega_i)\}_{i=1}^M$ will be passed into the discriminator, where their Wasserstein distance needs to be minimized. 
To simplify the notations for later use, we define $G_\theta: (\xi, B, \Tilde{X}) \mapsto X$ to represent the overall transformation in \eqref{eq:dc_sde-simulation}, with $\theta$ denoting all network parameters of $V_0$ and $V_1$.

%let $B$ to be the Brownian motions in \eqref{eq:dc_sde} and use the map $G_\theta: (\xi, B, \Tilde{X}) \mapsto X$ to represent the overall behavior of the neural DC-SDE generator.

{\bf Decorrelating and Branching Phase.}
During testing, we utilize a branching scheme to alleviate the independence problem; see Figure~\ref{fig:branch} for an illustrative example.
Let $q$ be the number of steps we ``walk'' along the directed chain. Here ``walking'' along the chain means: After we have finished the training (identified $V_0$ and $V_1$) phase, we start with the first chain (the grey one in Figure \ref{fig:branch}). We take real data as the first neighborhood $X_1$ to generate $X_2$ through the scheme \eqref{eq:dc_sde-simulation}, where $X_1$ takes the role of $\tilde X$ and $X_2$ takes the role of $X$. Then we use $X_2$ as the neighborhood to generate $X_3$, and repeat this procedure until we obtain $X_q$. By Theorem \ref{thm:dependence_decay}, $X_q$ and $X_1$ are asymptotically uncorrelated, as $q \to \infty$. We describe the pseudo-code in Algorithm~\ref{algo:testing} below for this decorrelating step. %We describe the pseudo-code in Algorithm~\ref{algo:testing} in Appendix~\ref{app:codes} for this decorrelating step. 

\begin{figure}[htpb]
    \centering
    \vspace{.05in}
    \includegraphics[width=0.4\textwidth]{figures/branching.png}
    \vspace{.1in}
    \caption{Branching Scheme. Let $q$ be the number of steps we ``walk'' along the directed chain. We take real data as the first neighborhood $X_1$ to generate $X_2$ through the scheme \eqref{eq:dc_sde-simulation}, where $X_1$ takes the role of $\tilde X$ and $X_2$ takes the role of $X$. Then we use $X_2$ as the neighborhood to generate $X_3$, and repeat this procedure until we obtain $X_q$. }
    \label{fig:branch}
\end{figure}

\begin{algorithm}
\caption{Generator in the Decorrelating and Branching}
\label{algo:testing}
\begin{algorithmic}
\STATE {\bfseries Input:} real data $\{\Tilde{X}(\omega_i)\}_{i=1}^M$, \# of steps  $q$, generator $G_\theta$;
\STATE {\bfseries Set} $\{X_{1}(\omega_i)\}_{i=1}^M :=\{\Tilde{X}(\omega_i)\}_{i=1}^M$;
\FOR{$k=2$ {\bfseries to} $q$}
\STATE Generate $M$ independent copies of initials positions and Brownian paths $\{\xi_k(\omega_i), B_k(\omega_i)\}_{i=1}^M$;
\STATE Generate $M$ paths $\{X_k(\omega_i)\}_{i=1}^M$ by $$X_k(\omega_i) = G_\theta(\xi_k(\omega_i), B_k(\omega_i), X_{k-1}(\omega_i));$$
\ENDFOR
\STATE {\bfseries Output:} $\{X_q(\omega_i)\}_{i=1}^M$ %, $k = 1, \ldots , q$. 
\end{algorithmic}
\end{algorithm}


To generate more fake data, we can initiate more chains with the same starting node $X_1$  (where the real data are) and independent Brownian paths, and then ``walk'' along the chain to get $X_q^{(i)}, i=2,3,\dots$. Again, $X_q^{(i)}$ is asymptotically uncorrelated to $X_1$. By the definition of DC-SDEs, $X_q$ and $X_q^{(i)}$ are conditionally independent with conditioning on $X_1$. Therefore, we can claim that $X_q$ and $X_q^{(i)}$ are asymptotically uncorrelated. 

%The detailed steps in testing phase can be summarized in Algorithm \ref{algo:testing}.




{\bf Architecture.} Note that although the directed chain SDE pair $(X, \Tilde{X})$ is Markovian, $X$ itself can be non-Markovian as a standalone stochastic process. All the historical information can be embedded in the neighborhood process and fetched through $V_0$ and $V_1$. Such a property leads to one of the key differences between our method and Neural SDEs: there is no need to embed time series into a hidden space. In our implementations, $V_0$ and $V_1$ take standard feedforward neural networks; see Appendix~\ref{app:experiment} for details.


\subsection{Discriminator}
The purpose of the discriminator is to identify the optimal parameters in the $V_0$- and $V_1$- networks. We use the Wasserstein GAN  framework \citep{goodfellow2020generative, arjovsky2017wasserstein} to train the generator, and two types of discriminators will be used here.

{\bf SigWGAN.} %Expected signature has been widely used to capture the distribution of sequential data. 
Using the idea of expected signature, \citet{ni2020conditional, ni2021sig} designed  Sig-Wasserstein GAN by directly minimizing the signature Wasserstein-1 distance,% defined by
\begin{equation*}
%\label{eq:sig_mmd_infinite}
\mathrm{Sig\mbox{-}W}_1(\mu, \nu):= |\EE_{X\sim\mu}[S(X)] - \EE_{X\sim\nu}[S(X)]|,
\end{equation*}
where $\mu$ and $\nu$ are two distributions of time series corresponding to real data and fake data, $S$ is the signature map, and $|\cdot|$ is the $l_2$ norm. For practical use,  we approximate the infinite sequence $S$ by truncating signatures up to some finite order $m$, i.e.,
\begin{equation}
\label{eq:sig_mmd}
\mathrm{Sig\mbox{-}W}^m_1(\mu,\nu):= |\EE_{\mu}[S^m(X)] - \EE_{\nu}[S^m(X)]|.
\end{equation}
The higher the truncation order $m$, the more information the signature can capture. However, the number of terms in the truncated signature will grow exponentially and become costly when the time series data is high-dimensional.

{\bf Neural CDEs.} Neural controlled differential equations are the second candidate for the discriminator when the underlying time series is of high dimension. This is also the discriminator used in \cite{kidger2021neural}. Let $D_\phi: X \mapsto R$ be a Neural CDE discriminator where $\phi$ denotes the network parameters. The training goal is to solve the following optimization problem for the generator
$$\min_{\theta} \EE_{\xi, B}\big[D_\phi\big(G_\theta(\xi, B, \Tilde{X})\big)\big],$$
and the following one for the discriminator
\begin{align}
\max_\phi \big\{ \EE_{\xi, B}\big[ D_\phi\big(G_\theta(\xi, B, \Tilde{X})\big)\big] - \EE_{\Tilde{X}}\big[D_\phi(\Tilde{X}) \big]\big\}. \label{eq:cde_wgan}
\end{align}
Compared to only using the Neural CDEs as the discriminator, we notice that a combination of Neural CDEs and lower-order signature Wasserstein-1 distance as the discriminator works better for the third numerical example below. That is, the generator is optimized with respect to
\begin{align}
\min_{\theta} \big\{ &\EE_{\xi, B}\big[D_\phi\big(G_\theta(\xi, B, \Tilde{X})\big)\big] \nonumber\\
& + \mathrm{Sig\mbox{-}W}^m_1\big(\Law(\Tilde{X}), \Law\big(G_\theta(\xi, B, \Tilde{X})\big)\big) \big\}.\label{eq:combined_loss}
\end{align}
Remark that DC-GANs can work with different discriminators, and here we choose to use neural CDEs and SigWGAN as the discriminators.
The pseudo-algorithm of the overall training strategy is summarized in Algorithm~\ref{algo:training}. %in Appendix~\ref{app:codes}.

%{\color{red} For the purpose of proving that as a generator, Neural DC-SDEs works with different discriminator, we consider two cases with neural CDE and SigWGAN as their discriminators respectively.}


\begin{algorithm}
\caption{The Training Phase}
\label{algo:training}
\begin{algorithmic}
\STATE {\bfseries Input:} real data $\{\Tilde{X}(\omega_i)\}_{i=1}^M$, boolean variable $cde$, total epochs $E$, signature truncation order $m$;
\FOR{$e=1$ {\bfseries to} $E$}
\STATE Generate independent copies of initials and Brownian motions $(\xi(\omega_i), B(\omega_i))_{i=1}^M$;
\STATE Generate fake data $\{X(\omega_i)\}_{i=1}^M$ by 
$$X(\omega_i) = G_\theta(\xi(\omega_i), B(\omega_i), \Tilde{X}(\omega_i));$$\vspace{-10pt}
\IF{$cde$ is True}
\STATE Compute the loss \eqref{eq:cde_wgan} and its gradients w.r.t. $\phi$;
\STATE Compute the loss \eqref{eq:combined_loss} and its gradients w.r.t. $\theta$;
\STATE Update $\theta$ by stochastic gradient descent optimiser;
\STATE Update $\phi$ by stochastic gradient ascent optimiser;
\ELSE
\STATE Compute the loss \eqref{eq:sig_mmd} and its gradients w.r.t. $\theta$;
\STATE Update $\theta$ by stochastic gradient descent optimiser;
\ENDIF
\ENDFOR
\STATE {\bfseries Output:} Generator $G_\theta$.
\end{algorithmic}
\end{algorithm}
%\rh{pseudo-code of the algorithm}

==> Neural Directed Chain SDEs as Generator for Exotic Time Series (icml)/tex/sde.tex <==
\section{DIRECTED CHAIN SDEs AND SIGNATURES}
In this section, we introduce two mathematical concepts that serve as the backbones of our algorithm: directed chain SDEs and signatures. {In Section~\ref{sec:dc-sde}, we identify the central issue of naively generating time series from true data using DC-SDEs: the non-independence of the true data and fake data (Problem~\ref{prob:independence}). Then we overcome the non-independence issue by Decoorelating and Branching Phase in Section~\ref{sec:generator}, and provide theoretical guarantees for this procedure (Theorem~\ref{thm:dependence_decay}).}


In the sequel, we shall use $X_s, X_t$ to denote the state of $X$ at time $s$ and $t$, respectively. With no subscript, e.g., by $X$, we mean the whole path from $t=0$ to $T$.





\subsection{Directed Chain SDEs (DC-SDEs)}\label{sec:dc-sde}
%In this part, we introduce the structure and mathematical properties of the Directed Chain SDEs briefly, please see \citep{detering2020directed, ichiba2022smoothness} for more details. 



%For each pair of index $(i, i+1)$ where $i\le n-1$, $X_{i+1}$ depends on $X_{i}$ and we say the $i$-th particle is the neighborhood of the $(i+1)$-th particle. In the end, the $n$-th particle affects the first one and we therefore get a circle. The dependence is determined in a homogeneous manner over the whole system of particles. Such a circular chain structure forces every node to be identically distributed. When $n$ goes to infinity, the circle chain is equivalently to a non-circular chain with the {\bf distribution constraint} (see Def \ref{def:dc_sde}) and we get our abstract Directed Chain SDE.


{The DC-SDEs are the limit of a system of $n$-coupled SDEs interacting homogeneously on a directed chain when $n$ goes to infinity. Below we will focus on DC-SDEs and defer the introduction of this limiting process to Appendix~\ref{app:prelim}.}
Under the general setup, DC-SDEs can be of McKean-Vlasov type where the coefficients have distributions as inputs, corresponding to the $n$-coupled system having mean-field interaction. In our proposed generator, it is sufficient to use the simple case mentioned above, DC-SDE without the mean-field interaction, as in the following definition. 

%In general, directed chain SDE can also be defined as non-linear, McKean-Vlasov type (mean-field interaction) under the general case, where the coefficients have the distributional inputs. However, we only need the easier case here, Directed Chain SDE without the mean-field interaction in our model. Fix a filtered probability space $(\Omega, \mc{F}, (\mc{F}_t)_{t \ge 0}, \PP)$ and a finite time horizon $[0, T]$, we have the following definition,
\begin{defn}[DC-SDEs]
\label{def:dc_sde}
Fix a filtered probability space $(\Omega, \mc{F}, (\mc{F}_t)_{t \ge 0}, \PP)$ and a finite time horizon $[0, T]$.
Let $(X, \tilde{X})$ with $X, \tilde{X}\in L^2(\Omega\times [0,T], \RR^N)$ be a pair of square-integrable stochastic processes satisfying
\begin{equation} \label{eq:dc_sde}
    X_t = \xi \hspace{-2pt} + \hspace{-3pt}\int_0^t V_0(s, X_s, \tilde{X}_s)\ud s +  \hspace{-3pt}\int_0^t V_1(s, X_s, \tilde{X}_s)\ud B_s,
\end{equation}
for $t\in [0,T]$, with the {distributional constraint}
\begin{equation} \label{eq:dc_sde_a}
    \Law(X_t, 0\le t\le T)= \Law(\tilde{X}_t, 0\le t\le T),
\end{equation}
where {Law($\cdot$)} {stands for the distribution}, $V_0\in \RR^N$ and $V_1\in\RR^{N\times d}$ are smooth coefficients satisfying Lipschitz and linear growth conditions, $B$ is a standard $d$-dimensional Brownian motion, and $X_0:=\xi$, $\tilde{X}$ and $B$ are assumed to be independent.
%independent of the initial state $X_0:=\xi$ and $\tilde{X}_\cdot$, and finally, $\xi$ is independent of $\tilde{X}$.
\end{defn}

%the DC-SDE

The existence of the solution to  \eqref{eq:dc_sde} and the weak uniqueness in the sense of distribution have been proved under the Lipschitz and linear growth assumptions on the coefficients in \citet{detering2020directed} for a simple case, and in \citet{ichiba2022smoothness} for a more general case. Moreover, with the smoothness of the solution under certain additional conditions posed on the coefficients (cf. \citet{ichiba2022smoothness}), we can derive a partial differential equation (PDE) for the marginal densities of the solution. 
Then, the associated PDEs lead to the following theorem: DC-SDEs have at least the same amount of flexibility as Neural SDEs. 
\begin{thm}
\label{thm:flexibility}
Under proper assumptions, for any $Y$ that satisfies a system of Markovian SDEs on $[0,T]$, there exists a unique solution to the DC-SDE \eqref{eq:dc_sde} with constraints \eqref{eq:dc_sde_a}, some $V_0$ and non-degenerate coefficients $V_1$, such that they have the same marginal distributions for all $t\in[0,T]$. %, which have the same marginal distributions as the corresponding SDEs. 
Here by degenerate, we mean that $V_i(t, x, \tilde{x}):=V_i(t, x),\, i\in\{0,1\}$, i.e., the coefficients have no dependence on neighborhood nodes at all. 
%\footnote{{\color{blue} (TI) i think i need some rewriting here, and will be back later}}
\end{thm}
We defer the proof of Theorem~\ref{thm:flexibility} to Appendix~\ref{app:flexibility}.

%\begin{proof}
%See Appendix~\ref{app:flexibility}.
%\end{proof}

%This is indeed our proposal after learning $V_0$ and $V_1$. 

Naturally, if $V_0$ and $V_1$ are known (or learned from data), one can take real data paths as $\tilde X$ in \eqref{eq:dc_sde} and straightforwardly generate paths of $X$ that have the same distribution as $\tilde X$ by the constraint \eqref{eq:dc_sde_a}. However, naively implementing this idea will lead to the following potential problems. 

%\recheck{See Section \ref{sec:model} and Appendix XX below for the implementation.} 

\begin{problem}[Lack of Independence]
\label{prob:independence}
%We notice that the DC-SDEs generator may possess two potential problems:
%\begin{enumerate}
%
    The distribution of the generated sequence crucially depends on the real data; Consequently, to avoid dependence, {a single real path can only be used once as $\tilde X$} to generate one path of $X$, and thus the number of the generated sequence has to be the same as that of the training data set in one run. 
%\end{enumerate}
\end{problem}
Note that a qualified generator should also be able to generate \emph{unlimited} independent data that does not depend on the original one. %To qualify as a generator, it should be able to generate unlimited independent data that is independent of the original one. 
%Intuitively, the Directed Chain SDEs take the real paths as input, it could then heavily mimic the original path. Such behavior results in an one-to-one relationship between real data and generated data. However, an ideal generator should be able to generate any number of sequential data independently of the original. 
%We then say the Directed Chain SDEs as a generator has the independence problem.
%\begin{problem}[Independence]
%\label{prob:independence}
%We point out that Directed Chain SDEs generator has two major problem,
%\begin{enumerate}
%    \item the distribution generated sequence is not independent of the training data.
%    \item the number of generated sequence must be the same as training data. \rh{why, to avoid introducing further correlation between fake data}
%\end{enumerate}
%\end{problem}
Fortunately, both problems mentioned above can be overcome by the idea behind the following theorem.
\begin{thm}
\label{thm:dependence_decay}
Under mild non-degeneracy conditions, the correlation between training data and generated data in DC-SDEs decays exponentially fast, as the distance increases on the chain. %\rh{where do you define the distance on the chain? in appendix or main paper?}
\end{thm}
%\begin{proof}
Due to the page limit, we give the formal statement of Theorem~\ref{thm:dependence_decay} with detailed proof in Appendix~\ref{app:dependence-decay}.%  due to the page limit.
%\end{proof}

We shall explain how to beat the independence problem during the implementation described in Section~\ref{sec:generator}. As shown in Appendix \ref{app:dependence-decay}, the introduction of independent Brownian motions to \eqref{eq:dc_sde} is the key to solving the independence problem. We shall also provide an extreme example (cf. Remark \ref{rem:degenerate_eg}) showing that without $\int V_1 \ud B$, the system \eqref{eq:dc_sde}--\eqref{eq:dc_sde_a} has only trivial (deterministic) solution. %to show the importance of $V_1$ and independent Brownian motions.



\subsection{Signature} \label{sec:SignatureDef}
The proposed method utilizes signature \citep{lyons2007differential}, a concept from rough path theory that we shall briefly introduce for completeness. As an infinitely graded sequence, the signature can be understood as a feature extraction technique for time series data with certain regularity conditions. Let $x: \Omega\times[0,T] \to \RR^N$ be a continuous random process, and denote the signature map by $S: x\mapsto S(x) \in T(\RR^N)$, where $T(\RR^N)$ is the tensor algebra defined on $\RR^N$. Then,
$$S(x):=(1, x^1,\cdots, x^i, \dots), \quad \text{and}$$
$$x^i = \int_{0<t_1<\cdots < t_i < T} \ud x_{t_1} \otimes\cdots \otimes \ud x_{t_i}.$$
Signature characterizes paths uniquely up to the tree-like equivalence, and the equivalence is removed if at least one dimension of the path is strictly increasing \citep{boedihardjo2016signature}. The concept has been applied to design machine learning methods, e.g., \citet{chevyrev2018signature, kidger2019deep, min2021signatured, ni2021sig, min2022convolutional,dyer2021approximate}. In practice, one needs to truncate the signature up to a finite order $M$, denoted by $S^M(x)=(1,x^1,\cdots,x^M)$. We will justify the truncation by the factorial decay property and discuss other theoretical properties of signature in Appendix \ref{app:sig_decay}.  

In addition, signature induces another powerful tool to characterize the distribution of random processes: the \emph{expected signatures}. It was proved by \citet{chevyrev2016characteristic} that expected signatures characterize the distribution of random processes uniquely, i.e., if $\EE[S(x)]=\EE[S(y)]$ and $\EE[S(x)]$ has an infinite radius of convergence, then $x$ and $y$ have the same distribution. 

%\rh{another paragraph for introducing signature?}
